ZeroForge: Feedforward Text-to-Shape Without 3D Supervision

Current state-of-the-art methods for text-to-shape generation either require supervised training using a labeled dataset of pre-defined 3D shapes, or perform expensive inference-time optimization of implicit neural representations. In this work, we present ZeroForge, an approach for zero-shot text-to-shape generation that avoids both pitfalls. To achieve open-vocabulary shape generation, we require careful architectural adaptation of existing feed-forward approaches, as well as a combination of data-free CLIP-loss and contrastive losses to avoid mode collapse. Using these techniques, we are able to considerably expand the generative ability of existing feed-forward text-to-shape models such as CLIP-Forge. We support our method via extensive qualitative and quantitative evaluations

==> extra.tex <==
% \begin{table}[t!]
% \setlength\extrarowheight{3pt}
% \newcommand{\tabincell}[2]{\begin{tabular}{@{}#1@{}}#2\end{tabular}}
% \centering
% \begin{tabular}{lcc||lcc}
% \toprule
% \textbf{Class Name} & \textbf{zero\_conv} & \textbf{regular} &
% \textbf{Class Name} & \textbf{zero\_conv} & \textbf{regular} \\
% \hline
% umbrella & \includegraphics[width=2cm,height=2cm,keepaspectratio]{results/voxel\_renderings/q=easy\_5\_with\_original\_lr=1e-05\_beta=200\_gpu=0\_baseline=False\_v=128\_k=2\_r=nvr+\_s=1\_init=og\_init\_zero\_conv\_c=0.01\_improved\_temp=50/umbrella\_0.05.npy\_.png} & \includegraphics[width=2cm,height=2cm,keepaspectratio]{results/voxel\_renderings/q=easy\_5\_with\_original\_lr=1e-05\_beta=200\_gpu=0\_baseline=False\_v=128\_k=2\_r=nvr+\_s=1\_init=og\_init\_c=0.01\_improved\_temp=50/umbrella\_0.05.npy\_.png} &

% table & \includegraphics[width=2cm,height=2cm,keepaspectratio]{results/voxel\_renderings/q=easy\_5\_with\_original\_lr=1e-05\_beta=200\_gpu=0\_baseline=False\_v=128\_k=2\_r=nvr+\_s=1\_init=og\_init\_zero\_conv\_c=0.01\_improved\_temp=50/table\_0.05.npy\_.png} & \includegraphics[width=2cm,height=2cm,keepaspectratio]{results/voxel\_renderings/q=easy\_5\_with\_original\_lr=1e-05\_beta=200\_gpu=0\_baseline=False\_v=128\_k=2\_r=nvr+\_s=1\_init=og\_init\_c=0.01\_improved\_temp=50/table\_0.05.npy\_.png} \\ \hline

% barbell & \includegraphics[width=2cm,height=2cm,keepaspectratio]{results/voxel\_renderings/q=easy\_5\_with\_original\_lr=1e-05\_beta=200\_gpu=0\_baseline=False\_v=128\_k=2\_r=nvr+\_s=1\_init=og\_init\_zero\_conv\_c=0.01\_improved\_temp=50/barbell\_0.05.npy\_.png} & \includegraphics[width=2cm,height=2cm,keepaspectratio]{results/voxel\_renderings/q=easy\_5\_with\_original\_lr=1e-05\_beta=200\_gpu=0\_baseline=False\_v=128\_k=2\_r=nvr+\_s=1\_init=og\_init\_c=0.01\_improved\_temp=50/barbell\_0.05.npy\_.png} &

% airplane & \includegraphics[width=2cm,height=2cm,keepaspectratio]{results/voxel\_renderings/q=easy\_5\_with\_original\_lr=1e-05\_beta=200\_gpu=0\_baseline=False\_v=128\_k=2\_r=nvr+\_s=1\_init=og\_init\_zero\_conv\_c=0.01\_improved\_temp=50/airplane\_0.05.npy\_.png} & \includegraphics[width=2cm,height=2cm,keepaspectratio]{results/voxel\_renderings/q=easy\_5\_with\_original\_lr=1e-05\_beta=200\_gpu=0\_baseline=False\_v=128\_k=2\_r=nvr+\_s=1\_init=og\_init\_c=0.01\_improved\_temp=50/airplane\_0.05.npy\_.png}  \\\hline

% \tabincell{l}{christmas\\tree} & \includegraphics[width=2cm,height=2cm,keepaspectratio]{results/voxel\_renderings/q=easy\_5\_with\_original\_lr=1e-05\_beta=200\_gpu=0\_baseline=False\_v=128\_k=2\_r=nvr+\_s=1\_init=og\_init\_zero\_conv\_c=0.01\_improved\_temp=50/Christmas tree\_0.05.npy\_.png} & \includegraphics[width=2cm,height=2cm,keepaspectratio]{results/voxel\_renderings/q=easy\_5\_with\_original\_lr=1e-05\_beta=200\_gpu=0\_baseline=False\_v=128\_k=2\_r=nvr+\_s=1\_init=og\_init\_c=0.01\_improved\_temp=50/Christmas tree\_0.05.npy\_.png} &

% boat & \includegraphics[width=2cm,height=2cm,keepaspectratio]{results/voxel\_renderings/q=easy\_5\_with\_original\_lr=1e-05\_beta=200\_gpu=0\_baseline=False\_v=128\_k=2\_r=nvr+\_s=1\_init=og\_init\_zero\_conv\_c=0.01\_improved\_temp=50/boat\_0.05.npy\_.png} & \includegraphics[width=2cm,height=2cm,keepaspectratio]{results/voxel\_renderings/q=easy\_5\_with\_original\_lr=1e-05\_beta=200\_gpu=0\_baseline=False\_v=128\_k=2\_r=nvr+\_s=1\_init=og\_init\_c=0.01\_improved\_temp=50/boat\_0.05.npy\_.png} \\ \hline


% knife & \includegraphics[width=2cm,height=2cm,keepaspectratio]{results/voxel\_renderings/q=easy\_5\_with\_original\_lr=1e-05\_beta=200\_gpu=0\_baseline=False\_v=128\_k=2\_r=nvr+\_s=1\_init=og\_init\_zero\_conv\_c=0.01\_improved\_temp=50/knife\_0.05.npy\_.png} & \includegraphics[width=2cm,height=2cm,keepaspectratio]{results/voxel\_renderings/q=easy\_5\_with\_original\_lr=1e-05\_beta=200\_gpu=0\_baseline=False\_v=128\_k=2\_r=nvr+\_s=1\_init=og\_init\_c=0.01\_improved\_temp=50/knife\_0.05.npy\_.png} &

% chair & \includegraphics[width=2cm,height=2cm,keepaspectratio]{results/voxel\_renderings/q=easy\_5\_with\_original\_lr=1e-05\_beta=200\_gpu=0\_baseline=False\_v=128\_k=2\_r=nvr+\_s=1\_init=og\_init\_zero\_conv\_c=0.01\_improved\_temp=50/chair\_0.05.npy\_.png} & \includegraphics[width=2cm,height=2cm,keepaspectratio]{results/voxel\_renderings/q=easy\_5\_with\_original\_lr=1e-05\_beta=200\_gpu=0\_baseline=False\_v=128\_k=2\_r=nvr+\_s=1\_init=og\_init\_c=0.01\_improved\_temp=50/chair\_0.05.npy\_.png} \\ \hline

% spoon & \includegraphics[width=2cm,height=2cm,keepaspectratio]{results/voxel\_renderings/q=easy\_5\_with\_original\_lr=1e-05\_beta=200\_gpu=0\_baseline=False\_v=128\_k=2\_r=nvr+\_s=1\_init=og\_init\_zero\_conv\_c=0.01\_improved\_temp=50/spoon\_0.05.npy\_.png} & \includegraphics[width=2cm,height=2cm,keepaspectratio]{results/voxel\_renderings/q=easy\_5\_with\_original\_lr=1e-05\_beta=200\_gpu=0\_baseline=False\_v=128\_k=2\_r=nvr+\_s=1\_init=og\_init\_c=0.01\_improved\_temp=50/spoon\_0.05.npy\_.png} &

% television & \includegraphics[width=2cm,height=2cm,keepaspectratio]{results/voxel\_renderings/q=easy\_5\_with\_original\_lr=1e-05\_beta=200\_gpu=0\_baseline=False\_v=128\_k=2\_r=nvr+\_s=1\_init=og\_init\_zero\_conv\_c=0.01\_improved\_temp=50/television\_0.05.npy\_.png} & \includegraphics[width=2cm,height=2cm,keepaspectratio]{results/voxel\_renderings/q=easy\_5\_with\_original\_lr=1e-05\_beta=200\_gpu=0\_baseline=False\_v=128\_k=2\_r=nvr+\_s=1\_init=og\_init\_c=0.01\_improved\_temp=50/television\_0.05.npy\_.png} \\
% \bottomrule
% \end{tabular}
% \caption{Shapes generated from ZeroForge after finetuning on 5 queries which were not seen in pre-training data (umbrella, barbell, Christmas tree, knife, spoon) and 5 which were (table, airplane, boat, chair, television). Here we use $\lambda_C=0.01$}
% \label{tab:5_with_original}
% \end{table}




% \begin{table}[t!]
% \centering
% \setlength\extrarowheight{3pt}
% \begin{tabular}{|c|c|c|c|c|}
% \hline
% \textbf{Class Name} & \textbf{$\lambda_c = 0.01, \tau=30$} & \textbf{$\lambda_c = 0.1, \tau=30$} & \textbf{$\lambda_c = 0.01, \tau=50$} & \textbf{$\lambda_c = 0.1, \tau=50$} \\
% \hline
% spoon & \includegraphics[width=2cm,height=2cm,keepaspectratio]{results/batch_2/c=0.01_temp=30/spoon_0.05.npy_.png} & \includegraphics[width=2cm,height=2cm,keepaspectratio]{results/batch_2/c=0.1_temp=30/spoon_0.05.npy_.png} & \includegraphics[width=2cm,height=2cm,keepaspectratio]{results/batch_2/c=0.01_temp=50/spoon_0.05.npy_.png} &\includegraphics[width=2cm,height=2cm,keepaspectratio]{results/batch_2/c=0.1_temp=50/spoon_0.05.npy_.png} \\
% \hline
% fork & \includegraphics[width=2cm,height=2cm,keepaspectratio]{results/batch_2/c=0.01_temp=30/fork_0.05.npy_.png} & \includegraphics[width=2cm,height=2cm,keepaspectratio]{results/batch_2/c=0.1_temp=30/fork_0.05.npy_.png} & \includegraphics[width=2cm,height=2cm,keepaspectratio]{results/batch_2/c=0.01_temp=50/fork_0.05.npy_.png} & \includegraphics[width=2cm,height=2cm,keepaspectratio]{results/batch_2/c=0.1_temp=50/fork_0.05.npy_.png} \\
% \hline
% knife & \includegraphics[width=2cm,height=2cm,keepaspectratio]{results/batch_2/c=0.01_temp=30/knife_0.05.npy_.png} & \includegraphics[width=2cm,height=2cm,keepaspectratio]{results/batch_2/c=0.1_temp=30/knife_0.05.npy_.png} & \includegraphics[width=2cm,height=2cm,keepaspectratio]{results/batch_2/c=0.01_temp=50/knife_0.05.npy_.png} &\includegraphics[width=2cm,height=2cm,keepaspectratio]{results/batch_2/c=0.1_temp=50/knife_0.05.npy_.png} \\
% \hline
% wineglass & \includegraphics[width=2cm,height=2cm,keepaspectratio]{results/batch_2/c=0.01_temp=30/wineglass_0.05.npy_.png} & \includegraphics[width=2cm,height=2cm,keepaspectratio]{results/batch_2/c=0.1_temp=30/wineglass_0.05.npy_.png} & \includegraphics[width=2cm,height=2cm,keepaspectratio]{results/batch_2/c=0.01_temp=50/wineglass_0.05.npy_.png} &\includegraphics[width=2cm,height=2cm,keepaspectratio]{results/batch_2/c=0.1_temp=50/wineglass_0.05.npy_.png} \\
% \hline
% \end{tabular}
% \caption{}
% \label{tab:contrast_ablation}
% \end{table}



% \subsection{Recreating ShapeNet}

% \begin{table}[t!]
% \centering
% \begin{tabular}{>{\centering\arraybackslash}m{3cm}>{\centering\arraybackslash}m{3cm}}
% \toprule[1.5pt]
% \textbf{Set 1} & \textbf{Set 2} \\ 
% \midrule
% Airplane                & Sofa                \\ 
% Bench                & Table                \\ 
% Cabinet                & Phone                \\ 
% Automobile                & Boat                \\ 
% Chair                &                         \\ 
% Monitor                &                         \\
% Lamp                &                         \\ 
% Loudspeaker                &                         \\ 
% Firearm                &                         \\ 
% \bottomrule
% \end{tabular}
% \caption{ShapeNet subsets}
% \label{table:ShapeSets}
% \end{table}

% \begin{table*}[h]
% \centering
% \setlength\extrarowheight{3pt}
% \begin{tabular}{>{\raggedleft\arraybackslash}m{0.53\linewidth} >{\raggedleft\arraybackslash}m{0.14\linewidth} >{\raggedleft\arraybackslash}m{0.23\linewidth}}
% \toprule[1.5pt]
% & \textbf{FID (Set 2)} & \textbf{FID (Set 1 $\cup$ Set 2)} \\ 
% \hline
% {ZeroForge Trained on Set2} & 3374 & 3352 \\
% {ZeroForge with ZeroConv Trained on Set2} & 3453 & 3503 \\
% {ZeroForge Trained on Set1 $\bigcup$ Set2} & 3833 & 3661 \\
% {ZeroForge with ZeroConv Trained on Set1 $\bigcup$ Set2} & 3521 & 3407 \\
% {CLIP-Forge Trained on Set1 } & 3837 & 3771 \\
% {ZeroForge with Random Initialization} &  &  \\
% {CLIPForge Trained on Set 1 $\bigcup$ Set 2} & 4125  & 3687 \\
% {CLIPForge Trained on Set 1} &   &  \\
% \bottomrule
% \end{tabular}
% \caption{FID Scores on ShapeNet Classes. \textcolor{red}{Need to bold best score.}}
% \label{table:ShapeSetsTransposed}
% \end{table*}

% We divide the ShapeNet data into two subsets of classes (shown in \tabref{table:ShapeSets}) and train a CLIP-Forge model~\citep{CLIP-Forge} on the data in the first subset. Using this initialization, we test whether ZeroForge can be used to learn the remaining classes without using the relevant shape data. This gives us a useful metric for ZeroForge's performance as we can compare the shapes it generates on the held-out classes with the ground-truth shape data. To do this, we use the Frechet Inception Distance (FID)~\citep{FID} used by \citet{CLIP-Forge}

% To properly define FID for ZeroForge's output distribution, we found it necessary to re-train the classifier used by \citet{CLIP-Forge} as it had only been trained on ShapeNet data which was oriented right side up whereas shapes generated by ZeroForge have no canonical orientation. We use the same classifier architecture as \citet{CLIP-Forge} but randomly rotate the shape data used during training. Doing this lowers the classifier's validation accuracy from $94\%$ to $88\%$. 
% We then use this classifier to get embeddings for both the ground truth ShapeNet data as well as the shapes generated by ZeroForge

% \begin{table}[h]
% \centering
% \setlength\extrarowheight{3pt}
% \begin{tabular}{|c|c|c|}
% \hline
% \textbf{Class Name} & \textbf{Zero\_conv} & \textbf{Regular} \\
% \hline
% umbrella & \includegraphics[width=2cm,height=2cm,keepaspectratio]{results/voxel\_renderings/q=easy\_5\_with\_original\_lr=1e-05\_beta=200\_gpu=0\_baseline=False\_v=128\_k=2\_r=nvr+\_s=1\_init=og\_init\_zero\_conv\_c=0.01\_improved\_temp=50/umbrella\_0.05.npy\_.png} & \includegraphics[width=2cm,height=2cm,keepaspectratio]{results/voxel\_renderings/q=easy\_5\_with\_original\_lr=1e-05\_beta=200\_gpu=0\_baseline=False\_v=128\_k=2\_r=nvr+\_s=1\_init=og\_init\_c=0.01\_improved\_temp=50/umbrella\_0.05.npy\_.png} \\
% \hline
% barbell & \includegraphics[width=2cm,height=2cm,keepaspectratio]{results/voxel\_renderings/q=easy\_5\_with\_original\_lr=1e-05\_beta=200\_gpu=0\_baseline=False\_v=128\_k=2\_r=nvr+\_s=1\_init=og\_init\_zero\_conv\_c=0.01\_improved\_temp=50/barbell\_0.05.npy\_.png} & \includegraphics[width=2cm,height=2cm,keepaspectratio]{results/voxel\_renderings/q=easy\_5\_with\_original\_lr=1e-05\_beta=200\_gpu=0\_baseline=False\_v=128\_k=2\_r=nvr+\_s=1\_init=og\_init\_c=0.01\_improved\_temp=50/barbell\_0.05.npy\_.png} \\
% \hline
% christmas tree & \includegraphics[width=2cm,height=2cm,keepaspectratio]{results/voxel\_renderings/q=easy\_5\_with\_original\_lr=1e-05\_beta=200\_gpu=0\_baseline=False\_v=128\_k=2\_r=nvr+\_s=1\_init=og\_init\_zero\_conv\_c=0.01\_improved\_temp=50/Christmas tree\_0.05.npy\_.png} & \includegraphics[width=2cm,height=2cm,keepaspectratio]{results/voxel\_renderings/q=easy\_5\_with\_original\_lr=1e-05\_beta=200\_gpu=0\_baseline=False\_v=128\_k=2\_r=nvr+\_s=1\_init=og\_init\_c=0.01\_improved\_temp=50/Christmas tree\_0.05.npy\_.png} \\
% \hline
% knife & \includegraphics[width=2cm,height=2cm,keepaspectratio]{results/voxel\_renderings/q=easy\_5\_with\_original\_lr=1e-05\_beta=200\_gpu=0\_baseline=False\_v=128\_k=2\_r=nvr+\_s=1\_init=og\_init\_zero\_conv\_c=0.01\_improved\_temp=50/knife\_0.05.npy\_.png} & \includegraphics[width=2cm,height=2cm,keepaspectratio]{results/voxel\_renderings/q=easy\_5\_with\_original\_lr=1e-05\_beta=200\_gpu=0\_baseline=False\_v=128\_k=2\_r=nvr+\_s=1\_init=og\_init\_c=0.01\_improved\_temp=50/knife\_0.05.npy\_.png} \\
% \hline
% spoon & \includegraphics[width=2cm,height=2cm,keepaspectratio]{results/voxel\_renderings/q=easy\_5\_with\_original\_lr=1e-05\_beta=200\_gpu=0\_baseline=False\_v=128\_k=2\_r=nvr+\_s=1\_init=og\_init\_zero\_conv\_c=0.01\_improved\_temp=50/spoon\_0.05.npy\_.png} & \includegraphics[width=2cm,height=2cm,keepaspectratio]{results/voxel\_renderings/q=easy\_5\_with\_original\_lr=1e-05\_beta=200\_gpu=0\_baseline=False\_v=128\_k=2\_r=nvr+\_s=1\_init=og\_init\_c=0.01\_improved\_temp=50/spoon\_0.05.npy\_.png} \\
% \hline
% table & \includegraphics[width=2cm,height=2cm,keepaspectratio]{results/voxel\_renderings/q=easy\_5\_with\_original\_lr=1e-05\_beta=200\_gpu=0\_baseline=False\_v=128\_k=2\_r=nvr+\_s=1\_init=og\_init\_zero\_conv\_c=0.01\_improved\_temp=50/table\_0.05.npy\_.png} & \includegraphics[width=2cm,height=2cm,keepaspectratio]{results/voxel\_renderings/q=easy\_5\_with\_original\_lr=1e-05\_beta=200\_gpu=0\_baseline=False\_v=128\_k=2\_r=nvr+\_s=1\_init=og\_init\_c=0.01\_improved\_temp=50/table\_0.05.npy\_.png} \\
% \hline
% airplane & \includegraphics[width=2cm,height=2cm,keepaspectratio]{results/voxel\_renderings/q=easy\_5\_with\_original\_lr=1e-05\_beta=200\_gpu=0\_baseline=False\_v=128\_k=2\_r=nvr+\_s=1\_init=og\_init\_zero\_conv\_c=0.01\_improved\_temp=50/airplane\_0.05.npy\_.png} & \includegraphics[width=2cm,height=2cm,keepaspectratio]{results/voxel\_renderings/q=easy\_5\_with\_original\_lr=1e-05\_beta=200\_gpu=0\_baseline=False\_v=128\_k=2\_r=nvr+\_s=1\_init=og\_init\_c=0.01\_improved\_temp=50/airplane\_0.05.npy\_.png} \\
% \hline
% boat & \includegraphics[width=2cm,height=2cm,keepaspectratio]{results/voxel\_renderings/q=easy\_5\_with\_original\_lr=1e-05\_beta=200\_gpu=0\_baseline=False\_v=128\_k=2\_r=nvr+\_s=1\_init=og\_init\_zero\_conv\_c=0.01\_improved\_temp=50/boat\_0.05.npy\_.png} & \includegraphics[width=2cm,height=2cm,keepaspectratio]{results/voxel\_renderings/q=easy\_5\_with\_original\_lr=1e-05\_beta=200\_gpu=0\_baseline=False\_v=128\_k=2\_r=nvr+\_s=1\_init=og\_init\_c=0.01\_improved\_temp=50/boat\_0.05.npy\_.png} \\
% \hline
% chair & \includegraphics[width=2cm,height=2cm,keepaspectratio]{results/voxel\_renderings/q=easy\_5\_with\_original\_lr=1e-05\_beta=200\_gpu=0\_baseline=False\_v=128\_k=2\_r=nvr+\_s=1\_init=og\_init\_zero\_conv\_c=0.01\_improved\_temp=50/chair\_0.05.npy\_.png} & \includegraphics[width=2cm,height=2cm,keepaspectratio]{results/voxel\_renderings/q=easy\_5\_with\_original\_lr=1e-05\_beta=200\_gpu=0\_baseline=False\_v=128\_k=2\_r=nvr+\_s=1\_init=og\_init\_c=0.01\_improved\_temp=50/chair\_0.05.npy\_.png} \\
% \hline
% television & \includegraphics[width=2cm,height=2cm,keepaspectratio]{results/voxel\_renderings/q=easy\_5\_with\_original\_lr=1e-05\_beta=200\_gpu=0\_baseline=False\_v=128\_k=2\_r=nvr+\_s=1\_init=og\_init\_zero\_conv\_c=0.01\_improved\_temp=50/television\_0.05.npy\_.png} & \includegraphics[width=2cm,height=2cm,keepaspectratio]{results/voxel\_renderings/q=easy\_5\_with\_original\_lr=1e-05\_beta=200\_gpu=0\_baseline=False\_v=128\_k=2\_r=nvr+\_s=1\_init=og\_init\_c=0.01\_improved\_temp=50/television\_0.05.npy\_.png} \\
% \hline
% \end{tabular}
% \caption{Shapes generated from ZeroForge after finetuning on 5 queries which were not seen in pre-training data (umbrella, barbell, Christmas tree, knife, spoon) and 5 which were (table, airplane, boat, chair, television). Here we use $\lambda_C=0.01$}
% \label{tab:5_with_original_2}
% \end{table}


% \begin{table}[h]
% \centering
% \begin{tabular}{|c|c|c|}
% \hline
% Class Name & zero\_conv & regular \\
% \hline
% umbrella & \includegraphics[width=2cm,height=2cm,keepaspectratio]{results/voxel_renderings/q=easy_5_with_original_lr=1e-05_beta=200_gpu=0_baseline=False_v=128_k=2_r=nvr+_s=1_init=og_init_zero_conv_c=0.1_improved_temp=50/umbrella_0.05.npy_.png} & \includegraphics[width=2cm,height=2cm,keepaspectratio]{results/voxel\_renderings/q=easy\_5\_with\_original\_lr=1e-05\_beta=200\_gpu=0\_baseline=False\_v=128\_k=2\_r=nvr+\_s=1\_init=og\_init\_c=0.1\_improved\_temp=50/umbrella\_0.05.npy\_.png} \\
% \hline
% barbell & \includegraphics[width=2cm,height=2cm,keepaspectratio]{results/voxel\_renderings/q=easy\_5\_with\_original\_lr=1e-05\_beta=200\_gpu=0\_baseline=False\_v=128\_k=2\_r=nvr+\_s=1\_init=og\_init\_zero\_conv\_c=0.1\_improved\_temp=50/barbell\_0.05.npy\_.png} & \includegraphics[width=2cm,height=2cm,keepaspectratio]{results/voxel\_renderings/q=easy\_5\_with\_original\_lr=1e-05\_beta=200\_gpu=0\_baseline=False\_v=128\_k=2\_r=nvr+\_s=1\_init=og\_init\_c=0.1\_improved\_temp=50/barbell\_0.05.npy\_.png} \\
% \hline
% Christmas tree & \includegraphics[width=2cm,height=2cm,keepaspectratio]{results/voxel\_renderings/q=easy\_5\_with\_original\_lr=1e-05\_beta=200\_gpu=0\_baseline=False\_v=128\_k=2\_r=nvr+\_s=1\_init=og\_init\_zero\_conv\_c=0.1\_improved\_temp=50/Christmas tree\_0.05.npy\_.png} & \includegraphics[width=2cm,height=2cm,keepaspectratio]{results/voxel\_renderings/q=easy\_5\_with\_original\_lr=1e-05\_beta=200\_gpu=0\_baseline=False\_v=128\_k=2\_r=nvr+\_s=1\_init=og\_init\_c=0.1\_improved\_temp=50/Christmas tree\_0.05.npy\_.png} \\
% \hline
% knife & \includegraphics[width=2cm,height=2cm,keepaspectratio]{results/voxel\_renderings/q=easy\_5\_with\_original\_lr=1e-05\_beta=200\_gpu=0\_baseline=False\_v=128\_k=2\_r=nvr+\_s=1\_init=og\_init\_zero\_conv\_c=0.1\_improved\_temp=50/knife\_0.05.npy\_.png} & \includegraphics[width=2cm,height=2cm,keepaspectratio]{results/voxel\_renderings/q=easy\_5\_with\_original\_lr=1e-05\_beta=200\_gpu=0\_baseline=False\_v=128\_k=2\_r=nvr+\_s=1\_init=og\_init\_c=0.1\_improved\_temp=50/knife\_0.05.npy\_.png} \\
% \hline
% spoon & \includegraphics[width=2cm,height=2cm,keepaspectratio]{results/voxel\_renderings/q=easy\_5\_with\_original\_lr=1e-05\_beta=200\_gpu=0\_baseline=False\_v=128\_k=2\_r=nvr+\_s=1\_init=og\_init\_zero\_conv\_c=0.1\_improved\_temp=50/spoon\_0.05.npy\_.png} & \includegraphics[width=2cm,height=2cm,keepaspectratio]{results/voxel\_renderings/q=easy\_5\_with\_original\_lr=1e-05\_beta=200\_gpu=0\_baseline=False\_v=128\_k=2\_r=nvr+\_s=1\_init=og\_init\_c=0.1\_improved\_temp=50/spoon\_0.05.npy\_.png} \\
% \hline
% table & \includegraphics[width=2cm,height=2cm,keepaspectratio]{results/voxel\_renderings/q=easy\_5\_with\_original\_lr=1e-05\_beta=200\_gpu=0\_baseline=False\_v=128\_k=2\_r=nvr+\_s=1\_init=og\_init\_zero\_conv\_c=0.1\_improved\_temp=50/table\_0.05.npy\_.png} & \includegraphics[width=2cm,height=2cm,keepaspectratio]{results/voxel\_renderings/q=easy\_5\_with\_original\_lr=1e-05\_beta=200\_gpu=0\_baseline=False\_v=128\_k=2\_r=nvr+\_s=1\_init=og\_init\_c=0.1\_improved\_temp=50/table\_0.05.npy\_.png} \\
% \hline
% airplane & \includegraphics[width=2cm,height=2cm,keepaspectratio]{results/voxel\_renderings/q=easy\_5\_with\_original\_lr=1e-05\_beta=200\_gpu=0\_baseline=False\_v=128\_k=2\_r=nvr+\_s=1\_init=og\_init\_zero\_conv\_c=0.1\_improved\_temp=50/airplane\_0.05.npy\_.png} & \includegraphics[width=2cm,height=2cm,keepaspectratio]{results/voxel\_renderings/q=easy\_5\_with\_original\_lr=1e-05\_beta=200\_gpu=0\_baseline=False\_v=128\_k=2\_r=nvr+\_s=1\_init=og\_init\_c=0.1\_improved\_temp=50/airplane\_0.05.npy\_.png} \\
% \hline
% boat & \includegraphics[width=2cm,height=2cm,keepaspectratio]{results/voxel\_renderings/q=easy\_5\_with\_original\_lr=1e-05\_beta=200\_gpu=0\_baseline=False\_v=128\_k=2\_r=nvr+\_s=1\_init=og\_init\_zero\_conv\_c=0.1\_improved\_temp=50/boat\_0.05.npy\_.png} & \includegraphics[width=2cm,height=2cm,keepaspectratio]{results/voxel\_renderings/q=easy\_5\_with\_original\_lr=1e-05\_beta=200\_gpu=0\_baseline=False\_v=128\_k=2\_r=nvr+\_s=1\_init=og\_init\_c=0.1\_improved\_temp=50/boat\_0.05.npy\_.png} \\
% \hline
% chair & \includegraphics[width=2cm,height=2cm,keepaspectratio]{results/voxel\_renderings/q=easy\_5\_with\_original\_lr=1e-05\_beta=200\_gpu=0\_baseline=False\_v=128\_k=2\_r=nvr+\_s=1\_init=og\_init\_zero\_conv\_c=0.1\_improved\_temp=50/chair\_0.05.npy\_.png} & \includegraphics[width=2cm,height=2cm,keepaspectratio]{results/voxel\_renderings/q=easy\_5\_with\_original\_lr=1e-05\_beta=200\_gpu=0\_baseline=False\_v=128\_k=2\_r=nvr+\_s=1\_init=og\_init\_c=0.1\_improved\_temp=50/chair\_0.05.npy\_.png} \\
% \hline
% television & \includegraphics[width=2cm,height=2cm,keepaspectratio]{results/voxel\_renderings/q=easy\_5\_with\_original\_lr=1e-05\_beta=200\_gpu=0\_baseline=False\_v=128\_k=2\_r=nvr+\_s=1\_init=og\_init\_zero\_conv\_c=0.1\_improved\_temp=50/television\_0.05.npy\_.png} & \includegraphics[width=2cm,height=2cm,keepaspectratio]{results/voxel\_renderings/q=easy\_5\_with\_original\_lr=1e-05\_beta=200\_gpu=0\_baseline=False\_v=128\_k=2\_r=nvr+\_s=1\_init=og\_init\_c=0.1\_improved\_temp=50/television\_0.05.npy\_.png} \\
% \hline
% \end{tabular}
% \caption{Shapes generated from ZeroForge after finetuning on 5 queries which were not seen in pre-training data (umbrella, barbell, Christmas tree, knife, spoon) and 5 which were (table, airplane, boat, chair, television). Here we use $\lambda_C=0.1$}
% \label{tab:my_label2}
% \end{table}

% \begin{figure}[t!]
% \centering
% \setlength\extrarowheight{3pt}
% \begin{tabular}{cc||cc}
% \toprule
% \textbf{Class Name} & \textbf{3D Object} &
% \textbf{Class Name} & \textbf{3D Object} \\
% \hline
% fork & \includegraphics[width=4cm,height=4cm,keepaspectratio]{results/batch_4/c=0.01_improved_temp=20/fork\_0.05.npy\_.png} &
% hammer & \includegraphics[width=4cm,height=4cm,keepaspectratio]{results/batch_4/c=0.01_improved_temp=20/hammer\_0.05.npy\_.png} \\ \hline
% knife & \includegraphics[width=4cm,height=4cm,keepaspectratio]{results/batch_4/c=0.01_improved_temp=20/knife\_0.05.npy\_.png} &
% mushroom & \includegraphics[width=4cm,height=4cm,keepaspectratio]{results/batch_4/c=0.01_improved_temp=20/mushroom\_0.05.npy\_.png} \\
% \hline
% pencil & \includegraphics[width=4cm,height=4cm,keepaspectratio]{results/batch_4/c=0.01_improved_temp=20/pencil\_0.05.npy\_.png} & 
% sandal & \includegraphics[width=4cm,height=4cm,keepaspectratio]{results/batch_4/c=0.01_improved_temp=20/sandal\_0.05.npy\_.png} \\ \hline
% screw & \includegraphics[width=4cm,height=4cm,keepaspectratio]{results/batch_4/c=0.01_improved_temp=20/screw\_0.05.npy\_.png} &
% screwdriver & \includegraphics[width=4cm,height=4cm,keepaspectratio]{results/batch_4/c=0.01_improved_temp=20/screwdriver\_0.05.npy\_.png} \\ \hline
% sombrero & \includegraphics[width=4cm,height=4cm,keepaspectratio]{results/batch_4/c=0.01_improved_temp=20/sombrero\_0.05.npy\_.png} &
% spoon & \includegraphics[width=4cm,height=4cm,keepaspectratio]{results/batch_4/c=0.01_improved_temp=20/spoon\_0.05.npy\_.png} \\ \hline
% wineglass & \includegraphics[width=4cm,height=4cm,keepaspectratio]{results/batch_4/c=0.01_improved_temp=20/wineglass\_0.05.npy\_.png} &
% umbrella & \includegraphics[width=4cm,height=4cm,keepaspectratio]{results/batch_4/c=0.01_improved_temp=20/umbrella\_0.05.npy\_.png} \\
% % wineglass & \includegraphics[width=4cm,height=4cm,keepaspectratio]{results/batch_4/c=0.01_improved_temp=20/thimble\_0.05.npy\_.png} \\
% \bottomrule
% \end{tabular}
% \medskip
% \caption{Samples from a ZeroForge model trained on 12 challenging and complex shape classes not seen in the original data distribution}
% \label{tab:6_with_original}
% \end{figure}
